Quantum Computation Using Large Spin Qudits

This dissertation explores quantum computation using qudits encoded into large spins, emphasizing the concept of quantum co-design to harness the unique capabilities of physical platforms for enhanced quantum information processing. First, we delve into the generation of high-fidelity universal gate sets for quantum computation with qudits. Leveraging principles from quantum optimal control, Rydberg physics, and the atomic structure of alkaline-earth atoms, we propose protocols for high-fidelity universal gate sets in the ground state of 87Sr with reasonable experimental parameters. Next, we analyze schemes to encode a qubit in the large spin qudits for fault-tolerant quantum computation (FTQC). By comprehending the most dominant noise in the physical system, we develop FTQC protocols that outperform the standard protocols. Finally, considering spin qudits for neutral atom quantum computation, we studied protocols for converting leakage errors to erasure errors resource efficiently. Also, we developed cooling methods for neutral atoms without destroying the quantum information.

==> abstract.tex <==
% the abstract

\begin{doublespace}
% This dissertation explores quantum computation using qudits  encoded into large spins, emphasizing the concept of quantum co-design to harness the unique capabilities of physical platforms for enhanced quantum information processing.  First, we delve into the generation of high-fidelity universal gate sets for quantum computation with qudits.  
% We first study the ability to implement unitary maps on states of the $I=9/2$ nuclear spin in \textsuperscript{87}Sr, a $d=10$  dimensional (qudecimal) Hilbert space, using quantum optimal control. 
% For implementing the single qudit gates we used  a combination of nuclear spin-resonance and a tensor AC-Stark shift, by solely modulating the phase of a radio-frequency magnetic field, the system is quantum controllable.  Alkaline earth atoms, such as \textsuperscript{87}Sr, have a very favorable figure-of-merit for such control due to narrow intercombination lines and the large hyperfine splitting in the excited states.
% We numerically study the quantum speed-limit, optimal parameters, and the fidelity of arbitrary state preparation and full SU(10) maps, including the presence of decoherence due to optical pumping induced by the light-shifting laser. We also study the use of robust control to mitigate some dephasing due to inhomogenieties  in the light shift.  We find that with an  rf-Rabi frequency of $\Omega_\text{rf}$ and 0.5\% inhomogeneity  in the the light shift we can prepare an arbitrary Haar-random state in a time  $T={4.5}\pi/\Omega_\text{rf}$  with average fidelity $\langle \mathcal{F}_\psi \rangle =0.9992$, and an arbitrary Haar-random SU(10) map in a time $T=24\pi/\Omega_\text{rf}$ with average fidelity $\langle \mathcal{F}_U \rangle = 0.9923$.
% For the  generation of two-qudit entangling quantum logic gates, we use two techniques in quantum optimal control.  We take advantage of both continuous, Lie algebraic control and digital, Lie group control. 
% In both cases, the key is access to a time-dependent Hamiltonian which can generate an arbitrary unitary matrix in the group SU($d^2$). 
% We find efficient protocols for creating high-fidelity entangling gates by manipulating the magnetic and optical fields, with entangling interactions arising from the well-known Rydberg blockade.
% Controlling the system through a combination of nuclear spin-resonance,  a tensor AC-Stark shift, and Rydberg dressing, which allows us to generate an arbitrary symmetric entangling two-qudit gate such as CPhase. 
% Our techniques can be used to implement qudit entangling gates for any  $2\le d \le 10$ encoded in the nuclear spin. We also studied how decoherence due to the finite lifetime of the Rydberg states affects the creation of the CPhase gate and found, through numerical optimization, a fidelity of $0.9985$, $0.9980$, $0.9942$, and $0.9800$ for $d=2$, $d=3$, $d=5$, and $d=7$  respectively.
% This provides a powerful platform to explore the various applications of quantum information processing of qudits including metrological enhancement with qudits, quantum simulation, universal quantum computation, and quantum error correction.

% Next we construct a fault-tolerant quantum error-correcting protocol based on a qubit encoded in a large spin qudit using a spin-cat code, analogous to the continuous variable cat encoding.
% With this, we can correct the dominant error sources, namely processes that can be expressed as error operators that are linear or quadratic in the components of angular momentum.  
% Such codes tailored to dominant error sources can exhibit superior thresholds and lower resource overheads when compared to those designed for unstructured noise models.
% A key component is the CNOT gate that preserves the rank of spherical tensor operators. 
% Categorizing the dominant errors as phase and amplitude errors, we demonstrate how phase errors, analogous to phase-flip errors for qubits, can be effectively corrected. Furthermore, we propose a  measurement-free error correction scheme to address amplitude errors without relying on syndrome measurements.
% Through an in-depth analysis of logical CNOT gate errors, we establish that the fault-tolerant threshold for error correction in the spin-cat encoding surpasses that of standard qubit-based encodings.
% We consider a specific implementation based on neutral-atom quantum computing, with qudits encoded in the nuclear spin of $^{87}$Sr, and show how to generate the universal gate set, including the rank-preserving CNOT gate, using quantum control and the Rydberg blockade. These findings pave the way for encoding a qubit in a large spin with the potential to achieve fault tolerance, high threshold, and reduced resource overhead in quantum information processing.


% Lastly, considering the qudit encoded in the ground space of $^{87}$Sr as a platform for neutral atom quantum computation, we studied  protocols for converting leakage errors to erasure errors resource efficiently. 
% For  neutral atom quantum computation, there is a finite probability of the information stored to be lost during quantum operations, this could be due to atoms escaping the trap or during the entangling interactions. 
% These errors in general known as leakage errors are detrimental for fault-tolerant quantum computation as they are not Pauli errors and need separate error correction protocols. 
% Another critical roadblock for quantum computation with neutral atoms is the lack of a cooling scheme while preserving the coherence, this in turn prevents us from doing arbitrarily long quantum computation. 
% In this work, we develop a scheme to cool the atoms while preserving the coherence without a very large magnetic field. 
% The scheme works for alkaline earth atoms where we store the quantum information in the nuclear spin. 
% For these atoms, one can use metastable states with narrow linewidth to employ the techniques of resolved sideband cooling. 
% To avoid mixing electronic and nuclear degrees of freedom in the excited state, which we need for cooling, we use Laser interaction which generates a fiducial magnetic field. 
% This decouples the electronic and nuclear degrees of freedom and avoids the ``which way information’’ about the nuclear spin state and one can cool while preserving coherence. These advances could significantly improve the prospect of neutral atoms for fault-tolerant quantum computation.

% % Leveraging principles from quantum optimal control, Rydberg physics, and the atomic structure of alkaline-earth atoms, we propose protocols for high-fidelity universal gate sets in the ground state of $^{87}$Sr with reasonable experimental parameters. Next, we analyze schemes to encode a qubit in the large spin qudits for fault-tolerant quantum computation (FTQC). By comprehending the most dominant noise in the physical system, we develop FTQC protocols that outperform the standard protocols. Finally, considering spin qudits for neutral atom quantum computation, we studied protocols for converting leakage errors to erasure errors resource efficiently. Also, we developed cooling methods for neutral atoms without destroying the quantum information.


This dissertation explores quantum computation using qudits encoded into large spins, emphasizing the concept of quantum co-design to harness the unique capabilities of physical platforms for enhanced quantum information processing.  First, we delve into the generation of high-fidelity universal gate sets for quantum computation with qudits. Leveraging principles from quantum optimal control, Rydberg physics, and the atomic structure of alkaline-earth atoms, we propose protocols for high-fidelity universal gate sets in the ground state of $^{87}$Sr with reasonable experimental parameters. Next, we analyze schemes to encode a qubit in the large spin qudits for fault-tolerant quantum computation (FTQC). By comprehending the most dominant noise in the physical system, we develop FTQC protocols that outperform the standard protocols. Finally, considering spin qudits for neutral atom quantum computation, we studied protocols for converting leakage errors to erasure errors resource efficiently. Also, we developed cooling methods for neutral atoms without destroying the quantum information.

\end{doublespace}

==> dedication.tex <==
%!TEX root = ../dissertation.tex
% dedication text
To my dear girlfriend and my greatest strength, Anu.


==> results_relax.tex <==
We now provide a high-level overview of the main contributions of this work. We provide summary cartoon in Figure~\ref{fig:quantum_classical_round_cartoon}, depicting the quantum embedding of the problem and the quantum rounding protocols. Let $(V, E)$ be a graph where we label the vertices by $V = [m]$, and denote the objective function of Problem~\eqref{eq:LNCG} by
\begin{equation}\label{eq:summary_obj}
    f(\mathbf{R}) \coloneqq \sum_{(u, v) \in E} \langle C_{uv}, R_u R_v^\T \rangle.
\end{equation}

\input{cartoon_figure_relax}

\subsection{Quantum Hamiltonian relaxation}

First, consider the setting in which $\mathbf{R} = (R_1, \ldots, R_m) \in \Orth(n)^m$. We embed this problem into a Hamiltonian by placing $n$ qubits on each vertex $v \in [m]$, resulting in a total Hilbert space $\mathcal{H}_{2^n}^{\otimes m}$ of $mn$ qubits. Define the $n$-qubit Pauli operators
\begin{equation}
    P_{ij} \coloneqq \begin{cases}
    -X_i Z_{i+1} \cdots Z_{j-1} X_j & i < j,\\
    Z_i & i = j,\\
    -Y_j Z_{j+1} \cdots Z_{i-1} Y_i & i > j,
    \end{cases}
\end{equation}
where $Z_i \coloneqq \I_2^{\otimes (i-1)} \otimes Z \otimes \I_2^{\otimes (n-i)}$ (similarly for $X_i$, $Y_i$). The Hamiltonian
\begin{equation}\label{eq:LNCG_H_summary}
    H \coloneqq \sum_{(u, v) \in E} \sum_{i, j \in [n]} [C_{uv}]_{ij} \sum_{k \in [n]} P_{ik}^{(u)} \otimes P_{jk}^{(v)}
\end{equation}
defines our quantum relaxation of the objective $f$ over $\Orth(n)^m$. The notation $A^{(v)}$ denotes the operator $A$ acting only on the Hilbert space of vertex $v$, and we overload this notation to indicate either the $n$-qubit operator or $mn$-qubit operator acting trivially on the remaining vertices. When the context is clear we typically omit writing the trivial support.

For optimization over $\SO(n)^m$, we consider instead the $(n-1)$-qubit Pauli operators
\begin{align}
    \widetilde{P}_{ij} &\coloneqq \Pi_0 P_{ij} \Pi_0^\T,\\
    \Pi_0 &= \frac{1}{\sqrt{2}} \l( \bra{+} \otimes \I_2^{\otimes (n-1)} + \bra{-} \otimes Z^{\otimes (n-1)} \r),
\end{align}
where $\Pi_0 : \mathcal{H}_{2^n} \to \mathcal{H}_{2^{n-1}}$ represents the projection onto the even-parity subspace of $\mathcal{H}_{2^n}$. The construction of the relaxed Hamiltonian for $\SO(n)$ is then analogous to Eq.~\eqref{eq:LNCG_H_summary}:
\begin{equation}
    \widetilde{H} \coloneqq \sum_{u, v \in E} \sum_{i, j \in [n]} [C_{uv}]_{ij} \sum_{k \in [n]} \widetilde{P}_{ik}^{(u)} \otimes \widetilde{P}_{jk}^{(v)},
\end{equation}
where now the relaxed quantum problem is defined over $m(n-1)$ qubits.

These Hamiltonians serve as relaxations to Problem~\eqref{eq:LNCG} in the following sense. First, we show that for every $R \in \Orth(n)$, there is an $n$-qubit state $\ket{\phi(R)}$ which is the maximum eigenstate of
\begin{equation}
    F(R) = \sum_{i,j \in [n]} R_{ij} P_{ij}.
\end{equation}
In particular, $F(R)$ is a free-fermion Hamiltonian, so $\ket{\phi(R)}$ is a fermionic Gaussian state. If $R \in \SO(n)$, then furthermore $\ket{\phi(R)}$ is an even-parity state, i.e., $\ev{\phi(R)}{Z^{\otimes n}}{\phi(R)} = 1$, so it is only supported on a subspace of dimension $2^{n-1}$ (the image of $\Pi_0$). This correspondence establishes a reformulation of the classical optimization problem as a constrained Hamiltonian problem:
\begin{equation}\label{eq:quantum_reformulation}
    \max_{\mathbf{R} \in G^m} f(\mathbf{R}) = \max_{\substack{\ket{\psi} = \bigotimes_{v \in [m]} \ket{\phi(R_v)} \\ R_v \in G}} \ev{\psi}{H}{\psi}.
\end{equation}
Dropping these constraints on $\ket{\psi}$ implies the inequalities
\begin{align}
    \max_{\mathbf{R} \in \Orth(n)^m} f(\mathbf{R}) &\leq \max_{\rho \in \mathcal{D}(\mathcal{H}_{2^n}^{\otimes m})} \tr(H \rho),\\
    \max_{\mathbf{R} \in \SO(n)^m} f(\mathbf{R}) &\leq \max_{\rho \in \mathcal{D}(\mathcal{H}_{2^{n-1}}^{\otimes m})} \tr(\widetilde{H} \rho),
\end{align}
where $\mathcal{D}(\mathcal{H})$ denotes the set of density operators on a Hilbert space $\mathcal{H}$. This establishes the quantum Hamiltonian relaxation.

\subsection{Quantum rounding}

\begin{algorithm}[t]
\caption{$\conv G$-based rounding of edge marginals.\label{alg:conv_rounding}}
\KwData{Quantum state $\rho \in \mathcal{D}(\mathcal{H}_d^{\otimes m})$ over a graph of $m$ vertices, each with local Hilbert space of dimension $d = 2^n$ if $G = \Orth(n)$, or $d = 2^{n-1}$ if $G = \SO(n)$}
\KwResult{Orthogonal matrices on each vertex, $R_1, \ldots, R_m \in G$}

$\mathcal{M} \gets \I_{mn}$ \;

\For{$u \neq v \in [m]$}{
    \For{$(i, j) \in [n]^2$}{
        \uIf{$G = \Orth(n)$}{
            $[\mathcal{M}_{uv}]_{ij} \gets \frac{1}{n} \tr(\Gamma_{ij}^{(u,v)} \rho)$ \;
        }
        \ElseIf{$G = \SO(n)$}{
            $[\mathcal{M}_{uv}]_{ij} \gets \frac{1}{n} \tr(\widetilde{\Gamma}_{ij}^{(u,v)} \rho)$ \;
        }
    }
}

\For{$v \in [m]$}{
    $R_v \gets \argmin_{Y \in G} \| Y - \mathcal{M}_{1v} \|_F$ \;
}
\end{algorithm}

\begin{algorithm}[t]

\caption{Rounding vertex marginals.\label{alg:vertex_rounding}}
\KwData{Quantum state $\rho \in \mathcal{D}(\mathcal{H}_d^{\otimes m})$ over a graph of $m$ vertices, each with local Hilbert space of dimension $d = 2^n$ if $G = \Orth(n)$, or $d = 2^{n-1}$ if $G = \SO(n)$}
\KwResult{Orthogonal matrices on each vertex, $R_1, \ldots, R_m \in G$}

\For{$v \in [m]$}{
    ${Q}_v \gets 0 \in \R^{n \times n}$ \;
    \For{$(i, j) \in [n]^2$}{
    \uIf{$G = \Orth(n)$}{
        $[{Q}_v]_{ij} \gets \tr(P_{ij}^{(v)} \rho)$ \;
    }
    \ElseIf{$G = \SO(n)$}{
        $[{Q}_v]_{ij} \gets \tr(\widetilde{P}_{ij}^{(v)} \rho)$ \;
    }
    }
}

\For{$v \in [m]$}{
    $R_v \gets \argmin_{Y \in G} \| Y - {Q}_v \|_F$ \;
}
\end{algorithm}

In order to recover orthogonal matrices from a relaxed quantum solution $\rho$, we propose two rounding procedures, summarized in Algorithms~\ref{alg:conv_rounding} and \ref{alg:vertex_rounding}. These rounding procedures operate on local (i.e., single- or two-vertex observables) expectation values of $\rho$ stored in classical memory, which can be efficiently estimated, e.g., by partial state tomography.

Algorithm~\ref{alg:conv_rounding} is inspired by constructing a quantum analogue of the PSD variable appearing in semidefinite relaxations to Problem~\eqref{eq:LNCG}. Consider the $mn \times mn$ matrix of expectation values
\begin{equation}
    \mathcal{M} \coloneqq \begin{bmatrix}
    \I_n & T_{12} & \cdots & T_{1m}\\
    T_{21} & \I_n & \cdots & T_{2m}\\
    \vdots & \vdots & \ddots & \vdots\\
    T_{m1} & T_{m2} & \cdots & \I_n
    \end{bmatrix},
\end{equation}
where the off-diagonal blocks are defined as
\begin{align}
    T_{uv} &\coloneqq \frac{1}{n} \begin{bmatrix}
    \tr(\Gamma_{11}^{(u, v)} \rho) & \cdots & \tr(\Gamma_{1n}^{(u, v)} \rho)\\
    \vdots & \ddots & \vdots\\
    \tr(\Gamma_{n1}^{(u, v)} \rho) & \cdots & \tr(\Gamma_{nn}^{(u, v)} \rho)
    \end{bmatrix} = T_{vu}^\T,\\
    \Gamma_{ij}^{(u, v)} &\coloneqq \sum_{k \in [n]} P_{ik}^{(u)} \otimes P_{jk}^{(v)}
\end{align}
when $G = \Orth(n)$, and we replace the operators $P_{ij}$ with $\widetilde{P}_{ij}$ when $G = \SO(n)$. We show that $\mathcal{M}$ satisfies the following properties for all states $\rho$:
\begin{align}
    &\mathcal{M} \succeq 0,\\
    &\mathcal{M}_{uv} \in \conv G \quad \forall u, v \in [m],
\end{align}
where $\conv G$ is the convex hull of $G$. Thus when $G = \SO(n)$, $\mathcal{M}$ obeys the same constraints as the $\conv\SO(n)$-based semidefinite relaxation proposed by Saunderson \emph{et al.}~\cite{saunderson2014semidefinite}. However, whereas the classical representation of the $\conv\SO(n)$ constraints requires at least matrices of size $2^{n-1} \times 2^{n-1}$ for each edge, our quantum state automatically satisfies these constraints (using only $n - 1$ qubits per vertex).

Algorithm~\ref{alg:vertex_rounding} uses the single-vertex information $\tr(P_{ij}^{(v)} \rho)$ of $\rho$, as opposed to the two-vertex information $\tr(\Gamma_{ij}^{(u, v)} \rho)$. We consider this rounding procedure due to the fact that, if $\rho$ is a pure Gaussian state satisfying the constraint of Eq.~\eqref{eq:quantum_reformulation}, then the matrix of expectation values
\begin{equation}
    Q_v \coloneqq \begin{bmatrix}
    \tr(P_{11}^{(v)} \rho) & \cdots & \tr(P_{1n}^{(v)} \rho)\\
    \vdots & \ddots & \vdots\\
    \tr(P_{n1}^{(v)} \rho) & \cdots & \tr(P_{nn}^{(v)} \rho)
    \end{bmatrix}
\end{equation}
lies in $\Orth(n)$. On the other hand, for arbitrary density matrices we have the relaxation $Q_v \in \conv\Orth(n)$, and again when we replace $P_{ij}^{(v)}$ with $\widetilde{P}_{ij}^{(v)}$ then $Q_v \in \conv\SO(n)$.

Both rounding procedures use the standard projection of the matrices $X \in \conv G$ (e.g., the matrices $T_{uv}$ or $Q_v$ measured from the quantum state) to some $R \in G$ by finding the nearest (special) orthogonal matrix according to Frobenius-norm distance:
\begin{equation}\label{eq:nearest_ortho_summary}
    R = \argmin_{Y \in G} \|X - Y\|_F.
\end{equation}
This can be solved efficiently as a classical postprocessing step, essentially by computing the singular value decomposition of $X = U \Sigma V^\T$. When $G = \Orth(n)$, the solution is $R = UV^\T$. When $G = \SO(n)$, we instead use the so-called special singular value decomposition of $X = U \widetilde{\Sigma} \widetilde{V}^\T$, where $\widetilde{\Sigma} = \Sigma J$ and $\widetilde{V} = VJ$, with $J$ being the diagonal matrix
\begin{equation}\label{eq:summary_J}
    J = \begin{bmatrix}
    \I_{n-1} & 0\\
    0 & \det(UV^\T)
    \end{bmatrix},
\end{equation}
assuming that the singular values $\sigma_i(X)$ are in descending order, $\sigma_1(X) \geq \cdots \geq \sigma_n(X)$. Then the solution to Eq.~\eqref{eq:nearest_ortho_summary} is $R = U \widetilde{V}^\T \in \SO(n)$.

==> thanks.tex <==
%!TEX root = ../dissertation.tex
% the acknowledgments section

During the whole journey leading up to this dissertation, I had the immense support of a large number of people.
First and foremost,  I would like to thank my advisor Ivan Deutsch for his support and guidance throughout my PhD.
Ivan is an incredible researcher and an amazing person. 
His passion for physics has always enthralled me and gave me insights into all the various facets of quantum information.
Also, his careful attention to developing communication skills has benefited me to a great extent.
Next, I would like to thank Milad Marvian, his amazing course is the sole reason that helped me understand the fundamental concepts of quantum error correction and develop some research directions.
His meticulous approach to research has also helped me in my research.
Also, Mike Martin has been an integral part of my research for the last four years. 
His valuable insights into the workings of the experiments have helped me in developing theoretical frameworks.
I would also like to thank Tameem Albash, who served as a member of my dissertation committee.



Next, I would like to thank Arul Lakshminarayan. 
He is the sole reason for my interest in the field of quantum information. 
He helped immensely during my Master's at IIT Madras both professionally and personally. 
I would like to thank Huayiu Duan whom I   had the chance to work with during the first two years at UNM.
Also, I had the chance to work with some outstanding people during my PhD.
In particular, I would like to thank Pablo Poggi, Jonathan Gross, Tyler Volkoff,  Ben Baragiola, Philip Blocher, Yuan-Yu Jau, and Tyler Thurtell.
All of them have helped me expand my understanding of the broader field of quantum information.



Also, I had the chance to interact with some amazing people in the field during my Ph.D.
I would like to thank Bethany, Saurbhav Panday, Hari Lamsal, Andrew Harter, Thomas Bersano,  Eric J. Meier, Noah Goss, and Long Nguyen for helping me understand the details of the experiments.
I also like to thank Charlie Baldwin, Josh Combes, Yale, Michael A. Perlin, Pranav Gokhale, Liang Jiang, David Heyes, Poul Jessen, Vaibhav Madhok, Prabha Mandayam, Nick Menicucci, Jun Ye, and Andreas Morella for some nice discussions.
Also, I would like to thank all the people and I forgot to acknowledge here. 

I want to thank the postdocs and my senior students at UNM, namely Gopi, Raf, Sayonee, Chris, Manuel, Karthik, Anupam, Sam, and Austin, for all their guidance throughout my time at UNM. 
Particularly, special thanks to Gopi, Anupam, and Karthik, who were very helpful when I first started working under Ivan and provided me with all the career advice. 
I am also grateful to all the graduate students in Ivan's group, Vikas, Andrew Forbes, Ivy, Mohsin, and Srinidhi whose support made this endeavor easier. 
I have benefited greatly from working with Vikas on multiple projects. 
 Finally, thanks to all of my friends and colleagues at CQuIC for the informative discussions and support:  Changhao, Andrew Zhao, Chaithanya, Benjamin Anker, Evan Borras, Zachary Castillo, Matthew Chow, Spencer Dimitroff, Cole K P, Cole Mauer, Shravan Shravan, and Jalan Ziyad.
 

I want to thank all my dear friends in Albuquerque for their support throughout my life here, namely Dave, Jayakrishnan, Sajay, Karthik, Savin, Desna, Vineeth, Veerendra, Aathira, Aswathy, Meenu, Lakshmi, Namitha, Jithin, Jerome, Sriram, Renjith, Aaditya, Johul, Srinath, Prashanth, Mahindra, Vinod, Nitin, Aadit, Hari, Jerin, Keerthana, Bertilla, and Catherine.
I also like to thank some of my friends who have been there with me for a long time, namely Azharu, Arjun, Sumit, Sangeeth, Jenet, Kevin, Jeena, Jithu, Govind, Anoop, Manoj, Akhil, Sachin, Arjun K Sabu, Hari, Anitta, Sunitha, Saranya, Gopika, and Ajith.

Also, I would like to thank my family who has been with me during this journey and for their constant support. 
Especially my father and mother for being there in each of my steps.
Also, my sister and my grandmother have given me amazing support even in my most stupid decisions.

Lastly, I would like to express my deepest gratitude to my amazing girlfriend, Anu Varghese, whose support has been invaluable. I met her during my Ph.D., and she has played an immense role in enriching my life over the past few years.
She has not only made me a better person but has also turned even the toughest of days into something beautiful.


